Mining Word Boundaries from Speech-Text Parallel Data for Cross-domain Chinese Word Segmentation

Inspired by early research on exploring naturally annotated data for Chinese Word Segmentation (CWS), and also by recent research on integration of speech and text processing, this work for the first time proposes to explicitly mine word boundaries from speech-text parallel data. We employ the Montreal Forced Aligner (MFA) toolkit to perform character-level alignment on speech-text data, giving pauses as candidate word boundaries. Based on detailed analysis of collected pauses, we propose an effective probability-based strategy for filtering unreliable word boundaries. To more effectively utilize word boundaries as extra training data, we also propose a robust complete-then-train (CTT) strategy. We conduct cross-domain CWS experiments on two target domains, i.e., ZX and AISHELL2. We have annotated about 1,000 sentences as the evaluation data of AISHELL2. Experiments demonstrate the effectiveness of our proposed approach.

==> tables/domain_adapt_latest_2024.7.tex <==

\begin{table*}[tb]
    \centering
    % \begin{small}
    
    % \setlength{\tabcolsep}{3.5pt}
    % \renewcommand{\arraystretch}{1.0}
    % \scalebox{0.7}{
    \begin{tabular}{lccccccc}
    \toprule 
    %% zx.no.punc
    % ~ & \multicolumn{3}{c}{ZX-dev} & \multicolumn{3}{c}{ZX-test} \\
    % \midrule
    % Models & P & R & F & P & R & F1 \\
    % \midrule
    % Baseline & 91.78 & 92.78 & 92.28 & 90.81 & 91.88 & 91.34 \\
    % CTT with \emph{ZX-SP} & 92.47 & 93.17 & \textbf{92.89} & 91.58 & 92.23 & {91.91} \\
    % CTT with \emph{All ZX-SP} & 92.58 & 93.19 & 92.88 & 91.66 & 92.23 & \textbf{91.95} \\
    % Self-training & 92.47 & 93.17 & 92.89 & 91.58 & 92.23 & 91.91 \\
    % \midrule
    %% zx.punc
    ~ & P & R & F1 & P & R & F1\\
    \midrule
    Models & \multicolumn{3}{c}{ZX-dev} & \multicolumn{3}{c}{ZX-test} \\
    
    \midrule
    Baseline & 94.16 & 94.39 & 94.27$_{\pm0.21}$ & 93.16 & 93.82 & 93.49$_{\pm0.22}$ \\    
    Using word boundaries & ~ & ~ & ~ & ~ & ~ & ~  \\
    \quad w/o filtering & 94.18 & 94.34 & 94.26$_{\pm0.49}$ & 93.69 & 94.03 & 93.86$_{\pm0.36}$ \\
    %Self-Training 
    \quad w/ filtering (${p}^\texttt{B} \geq 0.9$)
    & 94.27 & 94.64 & 94.45$_{\pm0.20}$ & 93.46 & 94.08 & {93.77}$_{\pm0.25}$ \\
    \quad w/ filtering (${p}^\texttt{B} \geq 0.1$) & 94.23 & 94.78 & \textbf{94.50}$_{\pm0.27}$ & 93.56 & 94.32 & \textbf{93.94}$_{\pm0.20}$ \\
    
    % \quad ${p} \geq 0.0$ & 93.69 & 94.03 & 93.86 \\
    % \quad ${p} \geq 0.1$ & 93.57 & 94.32 & \textbf{93.94} \\
    % \quad ${p} \geq 0.9$ & 93.46 & 94.08 & \underline{93.77} \\
    
    \midrule
    \multicolumn{7}{c}{Previous Results}  \\
    \midrule
    \citet{ding-etal-2020-coupling}  & ~ & ~ & --- & ~ & ~ &  90.90~~~~~~~~ \\
    \citet{luo-etal-2022-ji} & ~ & ~ & --- &  & ~ & 91.11~~~~~~~~ \\
    \citet{ShoheiHigashiyama2020}  & ~ & ~ & --- & ~ & ~ & 93.30~~~~~~~~ \\
    % \citet{jiang-etal-2021-fine}  & ~ & ~ & 95.07 \\
    
    \midrule
    \midrule

    Models & \multicolumn{3}{c}{AISHELL2-dev} & \multicolumn{3}{c}{AISHELL2-test} \\
    % \midrule
    % Models & P & R & F1 \\
    \midrule
    Baseline & 83.56 & 86.25 & 84.86$_{\pm1.55}$ & 86.11 & 88.94 & 87.48$_{\pm1.76}$ \\
    % % \midrule
    Using word boundaries & ~ & ~ & ~ & ~ & ~ & ~ \\
    \quad w/o filtering & 85.04 & 88.07 & 86.52$_{\pm1.07}$ & 86.29 & 89.21 & 87.71$_{\pm1.12}$  \\
    %Self-Training 
    \quad w/ filtering (${p}^\texttt{B} \geq 0.9$)
    & 85.38 & 87.87 & 86.60$_{\pm0.43}$ & 87.64 & 89.72 & {88.66}$_{\pm0.20}$ \\    
    % \quad w/ fitering (${p} \geq 0.1 and 0.3$) & 85.73 & 87.26 & \textcolor{red}{86.48}  & 88.58 & 89.83 & \textbf{89.19} \\    
    \quad w/ filtering (${p}^\texttt{B} \geq 0.1$) & 85.65 & 87.77 & \textbf{86.69}$_{\pm0.45}$ & 87.94 & 89.94 & \textbf{88.92}$_{\pm0.39}$ \\  

    

    \bottomrule % 表格底部粗横线
    \end{tabular}
    % }
    % \end{small}
    \caption{Main results on both datasets. 
    % The work of \citet{jiang-etal-2021-fine} introduces part-of-speech information for joint modeling.
    }
    \label{cross_domain}
    
\end{table*}

==> tables/natural_pauses.tex <==
\begin{table}[t]
    % \begin{small}
    \centering
    \setlength{\tabcolsep}{3.5pt}
    \renewcommand{\arraystretch}{1.1}
    \begin{tabular}{lrr}
    \toprule
    Item & ZX-unlabeled  & AISHELL2 \\
    \hline
    \# Sentences & 25,038 & 847,662 \\
    \# Sentences with \emph{SP} & 25,013 & 324,577 \\
    \# \emph{SP} & 179,397  & 537,986 \\
    % \# \emph{SP} & 203,842  & 537,986 \\
    \bottomrule 
    \end{tabular}
    % \caption{Statistics of data used in this paper.}  
    % \end{small}
    \caption{Statistics of unlabeled data. \emph{SP} is the abbreviation of Speech Pause.}  
    \label{total_data}
    
\end{table}


==> tables/pause_acc.tex <==
\begin{table}[tb]
    % \caption{Distribution of Pause Lengths in ZX-unlabeled and AISHELL2 datasets.}
    % \color{red}
    \begin{small}
    \centering
    \setlength{\tabcolsep}{3.5pt}
    \renewcommand{\arraystretch}{1.1}
    \begin{tabular}{lrrrr}
    \toprule 
    % ${[10,50)}$, ${[50,150)}$, ${[150,500)}$, and ${[500,)}$
    Duration ($\textit{ms}$) & 10-50 & 50-150 & 150-500 & 500-  \\
    % Duration ($\textit{ms}$) & ${[10,50)}$ & ${[50,150)}$ & ${[150,500)}$ &  ${[500,)}$  \\
    \midrule
    ~ & \multicolumn{4}{c}{ZX-unlabeled} \\
    \midrule
    Amount of pauses  & 9,281    & 20,840    & 87,326     & 61,950    \\
    Overall percent (\%) & 5.2  & 11.6     & 48.7    & 34.5  \\
    %Sampled pauses    & 320      & 1,331     & 5,677    & 3,096  \\
    Accuracy (\%)        & \underline{72.2} & 93.4  & 98.6   & 99.6  \\
    \midrule
    ~ & \multicolumn{4}{c}{AISHELL2} \\
    \midrule
    Amount of pauses   & 172,933  & 138,749   & 179,457    & 46,847 \\
    Overall percent (\%) & 32.1 & 25.8  & 33.4   & 8.7 \\ 
    \bottomrule % 表格底部粗横线
    \end{tabular}
    \end{small}
    \caption{Distribution of Pauses in ZX-unlabeled and AISHELL2 datasets. ``Overall percent'' denotes the proportion of pauses within a specific length interval relative to the total number of pauses. ``Sampled pauses'' denotes the quantity of samples from the current length interval.}
    \label{pause_acc}
    
\end{table}

